WINE: Wavelet-Guided GAN Inversion and Editing for High-Fidelity Refinement

Recent advanced GAN inversion models aim to convey high-fidelity information from original images to generators through methods using generator tuning or high-dimensional feature learning. Despite these efforts, accurately reconstructing image-specific details remains as a challenge due to the inherent limitations both in terms of training and structural aspects, leading to a bias towards low-frequency information. In this paper, we look into the widely used pixel loss in GAN inversion, revealing its predominant focus on the reconstruction of low-frequency features. We then propose WINE, a Wavelet-guided GAN Inversion aNd Editing model, which transfers the high-frequency information through wavelet coefficients via newly proposed wavelet loss and wavelet fusion scheme. Notably, WINE is the first attempt to interpret GAN inversion in the frequency domain. Our experimental results showcase the precision of WINE in preserving high-frequency details and enhancing image quality. Even in editing scenarios, WINE outperforms existing state-of-the-art GAN inversion models with a fine balance between editability and reconstruction quality.

==> fig/fig_inversion+editing.tex <==
\begin{figure*}[t]
\begin{center}
\includegraphics[width=0.95\textwidth]{res/fig_inversion+editing.pdf}
\end{center}
\caption{
\textbf{Qualitative comparison between inversion and editing results of baselines.}
In the inversion scenario from the first to third columns, The baseline models including the state-of-the-art high-rate inversion models failed to preserve details, such as accessories and complex backgrounds.
In contrast, inverted images through WINE showed robust reconstruction of image-wise details, \eg, legible letters on the third column.
We show edited images via InterFaceGAN from the fourth to eighth columns and editing results via StyleCLIP at the ninth and tenth columns.
Both low- and high-rate inversion baselines suffered from preserving details, \eg, letters, backgrounds, and hats.
HFGI, which relatively restored details among baselines, failed to edit the image in a disentangled way, \eg, distortion of eye shapes for editing with "beard".
Our proposed method effectively restored high-fidelity details with satisfactory editability with highly disentangled editing performance.
}
\label{fig:qualitative}
\end{figure*}


==> fig/fig_inversion_app.tex <==
\begin{figure*}[t]
\begin{center}
\includegraphics[width=\textwidth]{res/fig_inversion_app2.pdf}
\end{center}
\caption{
\textbf{Visualization of intermediate features during inversion.}
We visualize the intermediate output of our model for the inversion scenario.
$\hat\Delta$ indeed preserves image-specific details.
Consequently, $\hat{X}$ restores details that are missed in the low-rate inversion, \ie, $\hat{X}_{0}$, while maintaining the high perceptual quality.
Zoom in for a careful look into the details.
}
\label{fig:inversion_app}
\end{figure*}


==> fig/fig_visual.tex <==
\begin{figure*}[t]
\begin{center}
\includegraphics[width=0.9\textwidth]{res/fig_visual.pdf}
\end{center}
\caption{
\textbf{Qualitative comparison between inversion and editing results of baselines.}
From the first to the third rows, we show the inverted images. The inverted image from WINE preserves the most high-frequency details like the texture of clothes and skin. From the fourth to the seventh rows, we show edited images of various attributes via InterFaceGAN. WINE is the only method capable of editing images without loss of high-frequency information.}
\label{fig:appendix_visual}
\end{figure*}
\clearpage

==> sec/4_results.tex <==
% \input{fig/fig_inversion}
\input{fig/fig_editing}

\section{Experiments}
\label{experiments}


\noindent In this section, we compared the results of WINE with various GAN inversion methods.
We used the widely-used low-rate inversion models, \eg, $pSp$ \cite{richardson2021encoding},  $e4e$ \cite{tov2021designing}, and ReStyle \cite{alaluf2021restyle}, together with the state-of-the-art high-rate inversion models, \eg, HyperStyle \cite{alaluf2021hyperstyle}, HFGI \cite{wang2022high}, and StyleRes \cite{pehlivan2023styleres} as baselines.
First, we compared the qualitative results of inversion and editing scenarios. For editing, we used InterFaceGAN \cite{shen2020interfacegan} and StyleCLIP \cite{patashnik2021styleclip} to manipulate the latents.
Next, we compared the inversion performance quantitatively.
Finally, we analyzed the effectiveness of our wavelet loss and wavelet fusion through tactical ablation studies.
We first conducted experiments in the human face domain: we used Flickr-Faces-HQ (FFHQ) dataset \cite{karras2019style} for training and CelebA-HQ dataset \cite{Karras2018celeb} for evaluation, with all images generated to the high-resolution $1024^{2}$.  We trained our own $e4e$ encoder, InterFaceGAN, and StyleCLIP for each attribute to exploit the latent space of SWAGAN \cite{gal2021swagan}.
We also provide experimental results on Animal-Faces-HQ (AFHQ) dataset \cite{choi2020starganv2} additional ablation experimental results of WINE with varying fusion layers and fusion methods in supplementary material.
% in section \ref{sec:afhq}. 
% , and present the most optimal design for our model.


\noindent \textbf{Training Details.}
In our experiments, we implement our experiments based on the pytorch-version code \footnote{https://github.com/rosinality/stylegan2-pytorch} for SWAGAN \cite{gal2021swagan}.
% We converted the weights of pretrained SWAGAN generator checkpoint from the official tensorflow code\footnote{https://github.com/rinongal/swagan} to pytorch-version.
We trained our model on a single GPU and took only 6 hours for the validation loss to saturate, whereas other StyleGAN2-based baselines required more than 2 days of training time.

Here, we explain the details of our reconstruction loss terms: $\mathcal{L}_2$, $\mathcal{L}_{id}$, and $\mathcal{L}_{LPIPS}$. We leverage $\mathcal{L}_2$, as it is most effective in keeping the generated image similar to the original image pixel-wise.
$\mathcal{L}_{id}$ is an identity loss defined as:
\begin{equation}
    \mathcal{L}_{id} = 1-<R(G_0(w)), R(\mathbf{I}) > ,
\end{equation}
where $R$ is the pre-trained ArcFace \cite{deng2021arcface} model, and $\mathbf{I}$ is the ground truth image. $\mathcal{L}_{id}$ minimizes the cosine distance between two face images to preserve the identity. LPIPS \cite{zhang2018lpips} enhances the perceptual quality of the image by minimizing the distance on the feature space of ImageNet \cite{deng2009imagenet} pre-trained network.
For training, we used weights $\lambda_{\mathcal{L}_2}$=1,  $\lambda_{id}$=0.1, $\lambda_{LPIPS}$=0.8, respectively. 


\subsection{Qualitative Evaluation}
\label{exp:qual}

\input{tab/tab_inversion}

\noindent We first show the qualitative comparisons of inversions and editings in Figure \ref{fig:inversion} and Figure \ref{fig:editing}.  
We observed that our model produced more realistic inversion results than baselines, especially when images required more reconstructions of fine-grained details or complex backgrounds.
For instance, HyperStyle \cite{alaluf2021hyperstyle}, which refined weights of the generator per image, failed to reconstruct out-of-distribution objects, \eg, facial tattoo, and camera.
HFGI \cite{wang2022highcode} and StyleRes \cite{pehlivan2023styleres} could generate most of the lost details from the initial inversion, but restored details were close to artifacts, \eg, background letters.
In contrast, our method reconstructed details with minimum distortion consistently.

Figure \ref{fig:editing} shows editing results for six attributes, manipulated by InterFaceGAN \cite{shen2020interfacegan} and StyleCLIP \cite{patashnik2021styleclip}. 
Our model consistently showed the most robust results with high editability, while the baselines failed to either edit images or restore details.
For instance, in the case of InterFaceGAN, the baselines struggled to preserve details, \eg, the hats in the second to fourth rows.
% or showed low editability, \eg, HFGI in the sixth row.
In the case of StyleCLIP, the baselines similarly failed to preserve details, let alone address issues related to identity shifts.
% \eg, eyeglass at the sixth row, or showed undesirable entanglement, \eg, identity shift of HFGI, StyleRes at the sixth and seventh rows.
Overall, both InterFaceGAN and StyleCLIP editing results showed that our model is the most capable of handling the trade-off between reconstruction quality and editability.

\input{fig/fig_ablation}


\subsection{Quantitative Evaluation}
\noindent We evaluated inversion qualities with the existing baselines. Table \ref{tab:inversion} shows the quantitative results of each method. We used all images in the test split of CelebA-HQ and evaluated them with (i) the standard objectives including $\mathcal{L}_2$, LPIPS and ID similarity,
and (ii) the wavelet loss (equation \ref{eq:wavek}) to measure the spatial frequency distortion in the high-frequency sub-band.
Our model consistently outperformed every baseline by a large margin.
The results empirically prove that our wavelet loss and wavelet fusion in the frequency domain are capable of minimizing the distortion and thus improving the reconstruction quality.


\subsection{Ablation Study}
\label{sec:ablation}

\noindent In this section, we analyzed the effectiveness of each component of WINE, especially for our wavelet loss and wavelet fusion.
In Table \ref{tab:ablation}, we quantitatively compared the performance while changing each component.
We compared $\mathcal{L}_{1}$ through $\hat\Delta$ for the evaluation of $ADA$, and $\mathcal{L}_2$ and SSIM through $\hat X$ for the evaluation of the final inversion.

The \textbf{baseline} model without wavelets incorporated throughout the generator (StyleGAN2 \cite{karras2020analyzing}), and without our wavelet loss and wavelet fusion, corresponds to HFGI \cite{wang2022high}.
Firstly, configuration \textbf{A} only added the wavelet loss on HFGI.
We indeed found that the wavelet loss was helpful even when it was \textit{solely} used in the StyleGAN backbone.
In precise, \textsc{A} shows remarkably higher SSIM than HFGI.
Moreover, in Figure \ref{fig:ablation}, distortion in $\hat\Delta$ of \textsc{A} was decreased significantly, and details of $\hat X$ of \textsc{A}, \eg, fingers, were enhanced notably, compared to them of HFGI. For scenarios B to E, we adopted the generator with the hierarchical generation of wavelet coefficients (SWAGAN \cite{gal2021swagan}).
A simple modification of the generator from StyleGAN2 to SWAGAN (\textbf{B}) made marginal degradation in inversion.
We attribute this to the structure of existing inversion models, which are fitted to the StyleGAN.
In \textbf{C}, training with the wavelet loss achieved remarkably lower $\mathcal{L}_{1}(\Delta, \hat\Delta)$ (about 19\%) than training solely with $\mathcal{L}_{1}$.
Similar to A, this is compelling that training together with the wavelet loss achieved lower $\mathcal{L}_{1}$ than training solely with $\mathcal{L}_{1}$.
Moreover, as shown in Figure \ref{fig:ablation}, the wavelet loss was indeed helpful for preserving details, \eg, nail colors, compared to B.
With the residual transferred via wavelet fusion (\textbf{D}), though SSIM is improved, we can find ghosting artifacts in Figure \ref{fig:ablation}.
We assume that the absence of the wavelet loss refrains $ADA$ from finding the appropriate alignment, which leads to ghosting artifacts.
Finally, when \textbf{E} combined all the components together, \ie, WINE, apparent gain occurs on both $ADA$ and the final inversion.
Until \textsc{C}, though we elaborately calculated high-frequency features via wavelet loss, the model did not effectively transfer it to the generator.
The wavelet fusion at last enables the high-frequency information transfer to the generator, improving the inversion with the synergistic effect with wavelet loss.
The gains can be shown apparently in qualitative ways, as in Figure \ref{fig:ablation}.

\input{tab/tab_ablation}



